Interstellar extinction correction in ionised regions using HeI lines

The logarithmic extinction coefficient, c(H$\beta$), is usually derived using the H$\alpha$/H$\beta$ ratio for case B recombination and assuming standard values of electron density and temperature. However, the use of strong Balmer lines can lead to selection biases when studying regions with different surface brightness, such as extended nebulae, with the use of single integral field spectroscopy observations, since, in some cases, the H$\alpha$ line can be saturated in moderate to long exposures. In this work, we present a method to derive extinction corrections based only on the weaker lines of HeI, taking into account the presence of triplet states in these atoms and its influence on recombination lines. We have applied this procedure to calculate the extinction of different regions of the 30 Doradus nebula from MUSE integral-field spectroscopy data. The comparison between helium and hydrogen c(H$\beta$) determinations has been found to yield results fully compatible within the errors and the use of both sets of lines simultaneously reduces considerably the error in the derivation.

==> Tablas/Zamora-tab3.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline 
Line         & f($\lambda$) & F$_{obs}$          & I$^{line}_{teo}$/I$^{H\beta}_{teo}$& f($\lambda$)-f(H$\beta$) & log$_{10}$(F$^{line}_{obs}$/F$^{H\beta}_{obs}$) \\ \hline 

H$_{\alpha}$ & -0.313       & 1065613.0967845926 & 2.863157895      & -0.313                   & 0.65986222                                                          \\
H$_{\beta}$  & 0            & 233204.71650701217 & 1                & 0                        & 0                                                                   \\ 
Pa9          & -0.572       & 12831.189891480622 & 0.025433198      & -0.572                   & -1.259470397                                                        \\ 
Pa10         & -0.557       & 9030.127163293715  & 0.01842915       & -0.557                   & -1.412043464                                                        \\
Pa11         & -0.546       & 7172.850695271226  & 0.013789474      & -0.546                   & -1.512045539                                                        \\ 
Pa12         & -0.537       & 5584.2980064135    & 0.01059919       & -0.537                   & -1.620768743                                                        \\ 
Pa13         & -0.531       & 4074.5907615048727 & 0.008323887      & -0.531                   & -1.757653334                                                        \\ 
Pa14         & -0.525       & 3250.131162661459  & 0.006659919      & -0.525                   & -1.855836442                                                        \\ 
Pa15         & -0.521       & 2339.333804230504  & 0.005413765      & -0.521                   & -1.998645133                                                        \\ 
Pa16         & -0.518       & 1961.0739413215224 & 0.004460729      & -0.518                   & -2.075243361                                                        \\ 
Pa17         & -0.514       & 1539.2200181168748 & 0.003720648      & -0.514                   & -2.180436627                                                        \\ \hline
\end{tabular}
\caption{Medidas de las líneas de hidrógeno neutro en un espectro random.}
\end{table*}

==> Tablas/Zamora-tab4.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline 
Line              & f($\lambda$) & F$_{obs}$          & I$^{line}_{teo}$/I$^{HeI \lambda 6678}_{teo}$ & f($\lambda$)-f(He$\lambda$6678) & log$_{10}$(F$^{line}_{obs}$/F$^{HeI  \lambda 6678}_{obs}$) \\ \hline
HeI $\lambda$4922 & -0.014       & 2692.986167956774  & 0.344714856                                                   & 0.315                           & -0.676999399                                                              \\
HeI $\lambda$5875 & -0.209       & 37586.08179945757  & 3.518195753                                                   & 0.12                            & 0.467793532                                                               \\
HeI $\lambda$6678 & -0.329       & 12800.694185832053 & 1                                                             & 0                               & 0                                                                         \\
HeI $\lambda$7065 & -0.377       & 12989.322852250878 & 0.620997712                                                   & -0.048                          & 0.006352989                                                               \\
HeI $\lambda$7281 & -0.402       & 2483.683506520447  & 0.18696056                                                    & -0.073                          & -0.712137269                  \\ \hline                                          
\end{tabular}

\caption{Medidas de las líneas de helio neutro en un espectro random.}
\end{table*}

\begin{figure}
\begin{center}
\hspace{0.25cm}
\includegraphics[width=\columnwidth]{Zamora-fig4.png}
\caption{{\it Left:} [SIII]$\lambda$6312 map (240s). {\it Right:} [SIII]$\lambda$6312 map (2400s).}a
\end{center}
\end{figure}
\textcolor{red}{Fig. 3 shows that, in long exposure times observations (with H$\alpha$ lines saturated) we have been able to recover the information for smaller surface brightness areas by using the HeI lines.}

==> Tablas/Zamora-tab5.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|}
\hline 
Line              & f($\lambda$)$^a$& I$_\lambda$/I$_{H_\beta}$ $^b$\\ \hline
H$\alpha$ & -0.313 & 2.863\\
H$\beta$ & 0 & 1.000\\
Pa9 & -0.572 & 0.025\\
Pa10 & -0.557 & 0.018\\
Pa11 & -0.546 & 0.014\\
Pa12 & -0.537 & 0.011\\
Pa13 & -0.531 & 0.008\\
Pa14 & -0.525 & 0.007\\
Pa15 & -0.521 & 0.005\\
Pa16 & -0.518 & 0.004\\
Pa17 & -0.514 & 0.004\\ \hline 

\end{tabular}
\begin{tablenotes}
$^a$ \cite{1972ApJ...172..593M}, R$_v$ = 3.2 .\\ $^b$ \citet{pyneb}, n$_e$(cm$^{-3}$) = 10$^2$, T(K) = 10$^4$.
\end{tablenotes}
\caption{Teorical hydrogen values for the extinction curve and the ratio of lines.}
\end{table*}
